Constraints on the neutron star equation of state from AT2017gfo using radiative transfer simulations

The detection of the binary neutron star GW170817 together with the observation of electromagnetic counterparts across the entire spectrum inaugurated a new era of multi-messenger astronomy. In this study we incorporate wavelength-dependent opacities and emissivities calculated from atomic-structure data enabling us to model both the measured lightcurves and spectra of the electromagnetic transient AT2017gfo. Best-fits of the observational data are obtained by Gaussian Process Regression, which allows us to present posterior samples for the kilonova and source properties connected to GW170817. Incorporating constraints obtained from the gravitational wave signal obtained by the LIGO-Virgo Scientific Collaboration, we present a $90\%$ upper bound on the mass ratio $q \lesssim 1.38$ and a lower bound on the tidal deformability of $\tilde{\Lambda} \gtrsim 197$, which rules out sufficiently soft equations of state. Our analysis is a path-finder for more realistic kilonova models and shows how the combination of gravitational wave and electromagnetic measurements allow for stringent constraints on the source parameters and the supranuclear equation of state.

==> intro.tex <==
A new era of multi-messenger astronomy began with the combined detection of GW170817 \citep{AbEA2017b}, 
the gamma-ray burst (GRB) GRB170817A \citep{AbEA2017e}, and the electromagnetic transient 
AT2017gfo \citep{KiFo2017,SoHo2017,VaSa2017,ArHo2017,TaLe2017,LiGo2017}. 
This event proved that compact binary mergers including at least one neutron star 
can create an electromagnetic counterpart known as {\it kilonova}. 
The central engine of a kilonova are neutron-rich outflows which emit ultra-violet/optical/infrared 
emission powered by the radioactive decay of r-process elements \citep{LaSc1974,KaMe2017}. 
Kilonovae are of enormous scientific value, since they offer insight into 
the equation of state (EOS) of neutron stars \citep{BaBa2013,AbEA2017b,RaPe2018}, 
the formation of heavy elements \citep{JuBa2015,WuFe2016,RoLi2017}, 
and the expansion rate of the universe \citep{AbEA2017g}.

Because of their almost isotropic emission and bolometric luminosities of 
$\approx 10^{40}-10^{41}$\,ergs/s \citep{MeBa2015,BaKa2013} kilonovae are 
expected to be easily detectable with current telescopes \citep{MeBe2012}.
However, the optical signature of kilonovae depends on 
how matter was ejected from the merger and 
hence on details of the conditions at merger. 
Overall, there are two primary ejecta mechanism: dynamical ejecta and wind ejecta. 
The relative contribution of each depends on the source properties, 
including the binary mass ratio and the nuclear equation of state 
\citep{HoKi13,LeLi2016,RaGa2016,DiUj2017,SiMe2017,AbEA2017f}. 
The compositions of these ejecta also affect the emission from the system 
\citep{MeMa2010,KaBa2013,BaKa2013,TaHo2013,KaFe2015,BaKa2016,Me2017}. 
Neutron-rich ejecta generate an abundance of elements (A $>$ 130) that 
follows the Solar System r-process distribution \citep{KoRo2012,BaGo2013}.
Interestingly, the presence of Lanthanides and Actinides increases 
the optical opacity in the ejecta by orders of magnitudes  
relative to iron-group-like compositions, which results in dimmer, 
redder, and longer-lived optical/near-infrared emission \citep{KaBa2013}. 
Contrary, ejecta containing lighter r-process elements 
is expected to appear bluer and evolve faster \citep{FeMe2016}.

Dynamical ejecta become unbound around the moment of merger and 
travel with speeds 0.1-0.3\,c \citep{HoWa2016}. 
One the one hand, they can originate from torque during the merger leading to a quasi-toroidal geometry
and a low electron fraction due to the cold $\beta$-equilibrium in the original 
neutron star ($Y_e \approx 0.04$) \citep{RoFe2017}.
On the other hand, material gets dynamically ejected at the contact interface between the stars 
producing nearly isotropic geometries \citep{WoKo2017}. 
In the case where the interface ejecta is shock-heated or neutrino-irradiated, 
lighter r-process elements can be produced by ejecta with higher electron fractions \citep{WaSe2014},
but note that the levels of high electron fraction ejecta 
is still under debated due to its dependence on the EOS and on the neutrino physics 
\citep{SeKi2015,FoOc2015,PaLi2015,RoLi2017,LeLi2016,RaGa2016,FoOc2016}. 

Remnant accretion disk wind, driven by neutrino energy, magnetic fields, 
viscous evolution and/or nuclear recombination energy, is an additional source for ejecta \citep{MePi2008,DeOt2008,FeMe2013,PeRo2014,SiRi2014,JuBa2015,CiSi2015,MaSt2015}. 
It travels slower than the dynamical ejecta at velocity $\sim$\,0.05\,c.
Magnetically driven disk winds can contribute to outflows at either early or late times \citep{KiSe2015}. 
Furthermore, if there is sufficient neutrino irradiation from a hypermassive NS, 
outflows can be launched on the order of the thermal time, 
which is approximately 10-100\,ms post-merger, 
or $\geq 1$\,s on longer times when neutrino emission has 
ended and the disk reaches an advective 
state \citep{FeMe2013,JuBa2015,MePi2009,LeRa2009,FeMe2013}.

Since opacity and velocity control the diffusion time of the ejecta, 
the different ejecta channels have different characteristic magnitude, 
color, and durations. This is further complicated by the fact that the
observed color is viewing angle dependent \citep{KaFe2015}.
Finally, since dynamical ejecta can have a gravitationally bound component 
falling back onto the central object that can interact with the outflow and 
alter the mass ejection and composition of the disk. 
\cite{FeQu2015} showed that the disk outflow suppresses fallback accretion, 
and \cite{FeFo2017} extended this analysis by varying the relative mass ratios 
of the ejecta by changing the density of the dynamical ejecta.

With the detection of a kilonova optical counterpart to GW170817 there is significant interest in comparison to existing models of kilonova emission discussed above.
\cite{CoDi2017} showed how to use gravitational-wave and kilonova data together to perform parameter estimation of merger parameters.  In this paper, we build a parameterized surrogate model based on simulations from \cite{KaMe2017} and use it to infer the source properties of GW170817.  

